Program Synthesis using Abstraction Refinement

We present a new approach to example-guided program synthesis based on counterexample-guided abstraction refinement. Our method uses the abstract semantics of the underlying DSL to find a program $P$ whose abstract behavior satisfies the examples. However, since program $P$ may be spurious with respect to the concrete semantics, our approach iteratively refines the abstraction until we either find a program that satisfies the examples or prove that no such DSL program exists. Because many programs have the same input-output behavior in terms of their abstract semantics, this synthesis methodology significantly reduces the search space compared to existing techniques that use purely concrete semantics. While synthesis using abstraction refinement (SYNGAR) could be implemented in different settings, we propose a refinement-based synthesis algorithm that uses abstract finite tree automata (AFTA). Our technique uses a coarse initial program abstraction to construct an initial AFTA, which is iteratively refined by constructing a proof of incorrectness of any spurious program. In addition to ruling out the spurious program accepted by the previous AFTA, proofs of incorrectness are also useful for ruling out many other spurious programs. We implement these ideas in a framework called \tool. We have used the BLAZE framework to build synthesizers for string and matrix transformations, and we compare BLAZE with existing techniques. Our results for the string domain show that BLAZE compares favorably with FlashFill, a domain-specific synthesizer that is now deployed in Microsoft PowerShell. In the context of matrix manipulations, we compare BLAZE against Prose, a state-of-the-art general-purpose VSA-based synthesizer, and show that BLAZE results in a 90x speed-up over Prose.

==> casestudy.tex <==
\section{Case Studies}

In this section, we present two case studies to demonstrate how to instantiate our framework into two different application domain. 
The first case study is to automatically synthesize string transformations from input-output examples, a task that has been addressed in previous work~\cite{flashfill, blinkfill}. The second case study is to automatically learn programs that can perform tensor reshaping tasks, which is a new application. 
For each case study, we show how to instantiate our framework by providing a suitable DSL and the abstract semantics of the DSL constructs. 


\subsection{String Transformation}

We use the DSL from the most recent work~\cite{blinkfill}. In particular, the DSL is shown in \figref{stringdsl}. 






The abstract semantics of the DSL constructs is shown in \figref{stringdslasemantics}. 


\begin{figure}
\footnotesize  
\[
\begin{array}{rll}
\asemantics{\texttt{ConstPos}( r = c )} & \assign & \big( r = \semantics{\texttt{ConstPos}(c)} \big) \\ \\ 
\asemantics{\texttt{Pos}( \tau = c_1, k = c_2, d = c_3 )} & \assign & \big( p = \semantics{\texttt{Pos}(c_1, c_2, c_3)} \big) \\ \\ 
\asemantics{\texttt{SubStr}( x = c_1, p_1 = c_2, p_2 = c_3 )} & \assign & \big( f = \semantics{\texttt{SubStr}( c_1, c_2, c_3 )} \big) \\ \\ 
\asemantics{\texttt{ConstStr}( l = c )} & \assign & \big( l = \semantics{\texttt{ConstStr}( c )} \big) \\ \\ 
\asemantics{\texttt{Concat}( \emph{len}(f) = c_1, \emph{len}(e) = c_2 )} & \assign & \big( \emph{len}(e) = ( c_1 + c_2 ) \big) \\ 
\asemantics{\texttt{Concat}( \emph{len}(f) = c_1, e[c_2] = c_3 )} & \assign & \big( e[c_1 + c_2] = c_3 \big) \\ 
\asemantics{\texttt{Concat}( \emph{len}(f) = c_1, e = c_2 )} & \assign & \big( \emph{len}(e) = (c_1 + c_2) \wedge \bigwedge_{i = 0, \dots, c_2.\emph{len} - 1}{e[c_1.\emph{len} + i] = c_2[i]} \big) \\ 
\asemantics{\texttt{Concat}( f[c_1] = c_2, \emph{len}(e) = c_3 )} & \assign & \big( e[c_1] = c_2 \big) \\ 
\asemantics{\texttt{Concat}( f[c_1] = c_2, e[c_3] = c_4 )} & \assign & \big( e[c_1] = c_2 \big) \\ 
\asemantics{\texttt{Concat}( f[c_1] = c_2, e = c_3 )} & \assign & \big( e[c_1] = c_2 \big) \\ 
\asemantics{\texttt{Concat}( f = c_1, \emph{len}(e) = c_2 )} & \assign & \big( \emph{len}(e) = (c_1.\emph{len} + c_2) \wedge \bigwedge_{i = 0, \dots, c_1.\emph{len} - 1}{e[i] = c_1[i]} \big) \\ 
\asemantics{\texttt{Concat}( f = c_1, e[c_2] = c_3 )} & \assign & \big( e[c_1.\emph{len} + c_2] = c_3 \wedge \bigwedge_{i = 0, \dots, c_1.\emph{len} - 1}{e[i] = c_1[i]} \big) \\ 
\asemantics{\texttt{Concat}( f = c_1, e = c_2 )} & \assign & \big( e = \semantics{\texttt{Concat}(c_1, c_2)} \big) \\ 
\asemantics{\texttt{Concat}( \bigwedge_{i}{\pred_i}, \bigwedge_{j}{\pred_j} )} & \assign & \bigsqcap_{i} \bigsqcap_{j} \asemantics{\texttt{Concat}(\pred_i, \pred_j)} \\ \\ 
\asemantics{\texttt{Str}( \aval )} & \assign & \aval \\ \\ 
\end{array}
\]
\caption{Abstract semantics for string transformation DSL.}
\figlabel{stringdslasemantics}
\end{figure}


The universe $\universe$ is $\{ x = c, d = 0, d = 1, l = c, \tau = c, k = -3, \dots, k = 3, r = 0, \dots, r = 20, p = c, \emph{len}(f) = c, f[c_1] = c_2, f = c, \emph{len}(e) = c, e[c_1] = c_2, e = c, \emph{true}  \}$. 

The initial abstraction is 
$\{ x = c, d = 0, d = 1, l = c, \tau = c, k = -3, \dots, k = 3, r = 0, \dots, r = 20, p = c, \emph{len}(f) = c, \emph{len}(e) = c, \emph{true} \}$.


\subsection{Tensor Reshaping}

We use the DSL shown in \figref{matrixdsl}. It includes four important MATLAB functions that are used to perform matrix reshaping as following. 
\begin{itemize}
\item 
$\texttt{Reshape}(e, v)$: https://www.mathworks.com/help/matlab/ref/reshape.html 
\item 
$\texttt{Permute}(e, o)$: https://www.mathworks.com/help/matlab/ref/permute.html 
\item 
$\texttt{Fliplr}(e)$: https://www.mathworks.com/help/matlab/ref/fliplr.html 
\item 
$\texttt{Flipud}(e)$: https://www.mathworks.com/help/matlab/ref/flipud.html
\end{itemize}

In particular, in our DSL, we limit the vectors $o$ and $v$ of size at most 4. That means, we only consider tensors that have at most 4 dimensions. 

\begin{example}
https://stackoverflow.com/questions/23047184/how-to-reshape-a-cube-into-one-matrix-in-matlab
\end{example}


A tensor $e$ can be modeled as two vectors, $e.\emph{arr}$ and $e.\emph{size}$. The first vector $e.\emph{arr}$ is an array of elements in $e$ in column-wise manner. The second vector $e.\emph{size}$ denotes the size of $e$. 
For example, consider the matrix $e = [1,2,3;4,5,6]$, i.e., the first row is $[1,2,3]$ and the second row is $[3,4,5]$. We have $e.\emph{arr} = [1,4,2,5,3,6]$ and $e.\emph{size} = [2,3]$. 

The universe $\universe$ is $\{ l = c, k = c, o = c, \emph{len}(v) = c, v = c, \emph{len}(e.\emph{size}) = c, \emph{len}(e.\emph{arr}) = c, e = c, \emph{true} \}$. 

The initial abstraction $\preds$ is $\{ l = c, k = c, o = c, \emph{true} \}$.


\begin{figure}
\small 
\[
\begin{array}{rrll}
\text{Tensor} & e & \assign & \texttt{id}(x) \ | \ \texttt{Reshape}(e, v) \ | \ \texttt{Permute}(e, o) \ | \ \texttt{Fliplr}(e) \ | \ \texttt{Flipud}(e); \\  
\text{vector} & v & \assign & [k_1, k_2] \ | \ \texttt{Prepend}(k, v); \\ 
\text{vector} & o & \assign & [l_1, l_2] \ | \ \texttt{Prepend}(l, v); \\ 
\text{int} & k & \assign & 1 \ | \ \dots \ | \ 20; \\
\text{int} & l & \assign & 1 \ | \ 2 \ | \ 3 \ | \ 4; \\ 
\end{array}
\]
\caption{DSL fro tensor reshaping.}
\figlabel{matrixdsl}
\end{figure}



\begin{figure}
\footnotesize  
\[
\begin{array}{rll}
\asemantics{[ l_1 = c_1, l_2 = c_2 ]} & \assign & \big( o = \semantics{[c_1, c_2]} \big) \\ \\ 
\asemantics{\texttt{Prepend}( l = c_1, v = c_2 )} & \assign & \big( o = \semantics{\texttt{Prepend}(c_1, c_2)} \big) \\ \\ 
\asemantics{[ k_1 = c_1, k_2 = c_2 ]} & \assign & \big( v = \semantics{[c_1, c_2]} \big) \\ \\ 
\asemantics{\texttt{Prepend}( k_1 = c_1, \emph{len}(v) = c_2 )} & \assign & \big( \emph{len}(v) = (c_2 + 1) \wedge v[0] = c_1 \big) \\ 
\asemantics{\texttt{Prepend}( k_1 = c_1, v = c_2 )} & \assign & \big( v = \semantics{\texttt{Prepend}( c_1, c_2 )} \big) \\ \\ 
\asemantics{\texttt{id}( x = c )} & \assign & \big( x = \semantics{\texttt{id}( c )} \big) \\ \\ 
\asemantics{\texttt{Permute}( \emph{len}(e.\emph{size}) = c_1, o = c_2 )} & \assign & \big( \emph{len}(e.\emph{size}) = c_2.\emph{len} \big) \\ 
\asemantics{\texttt{Permute}( \emph{len}(e.\emph{arr}) = c_1, o = c_2 )} & \assign & \big( \emph{len}(e.\emph{arr}) = c_1 \wedge \emph{len}(e.\emph{size}) = c_2.\emph{len} \big) \\ 
\asemantics{\texttt{Permute}( e = c_1, o = c_2 )} & \assign & \big( e = \semantics{\texttt{Permute}( c_1, c_2 )} \big) \\ 
\asemantics{\texttt{Permute}( \bigwedge_{i}{\pred_i}, o = c )} & \assign & \bigsqcap_{i}{\asemantics{\texttt{Permute}( \pred_i, o = c )}}  \\ \\ 
\asemantics{\texttt{Reshape}( \emph{len}(e.\emph{size}) = c_1, \emph{len}(v) = c_2 )} & \assign & \big( \emph{len}(e.\emph{size}) = c_2 \big) \\ 
\asemantics{\texttt{Reshape}( \emph{len}(e.\emph{size}) = c_1, v = c_2 )} & \assign & \big( \emph{len}(e.\emph{size}) = c_2.\emph{len} \big) \\ 
\asemantics{\texttt{Reshape}( \emph{len}(e.\emph{arr}) = c_1, \emph{len}(v) = c_2 )} & \assign & \big( \emph{len}(e.\emph{arr}) = c_1 \wedge \emph{len}(e.\emph{size}) = c_2 \big) \\ 
\asemantics{\texttt{Reshape}( \emph{len}(e.\emph{arr}) = c_1, v = c_2 )} & \assign & \big( \emph{len}(e.\emph{arr}) = c_1 \wedge \emph{len}(e.\emph{size}) = c_2.\emph{len} \big) \\ 
\asemantics{\texttt{Reshape}( e = c_1, \emph{len}(v) = c_2 )} & \assign & \big( \emph{len}(e.\emph{arr}) = c_1.\emph{len} \wedge \emph{len}(e.\emph{size}) = c_2 \big) \\ 
\asemantics{\texttt{Reshape}( e = c_1, v = c_2 )} & \assign & \big( e = \semantics{\texttt{Reshape}(c_1, c_2)} \big) \\ 
\asemantics{\texttt{Reshape}( \bigwedge_{i}{\pred_i}, \bigwedge_{j}{\pred_j} )} & \assign & \bigsqcap_{i} \bigsqcap_{j} {\asemantics{\texttt{Reshape}( \pred_i, \pred_j )}} \\ \\  
\end{array}
\]
\[
\begin{array}{ll}
\begin{array}{rll}
\asemantics{\texttt{Flipud}( \emph{len}(e.\emph{size}) = c )} & \assign & \big( \emph{len}(e.\emph{size}) = c \big) \\ 
%\asemantics{\texttt{Flipud}( e.\emph{size}[c_1] = c_2 )} & \assign & \big( e.\emph{size}[c_1] = c_2 \big) \\ 
\asemantics{\texttt{Flipud}( \emph{len}(e.\emph{arr}) = c )} & \assign & \big( \emph{len}(e.\emph{arr}) = c \big) \\ 
%\asemantics{\texttt{Flipud}( e.\emph{arr}[c_1] = c_2 )} & \assign & \emph{true} \\ 
\asemantics{\texttt{Flipud}( e = c )} & \assign & \big( e = \semantics{\texttt{Flipud}(c)} \big) \\ 
\asemantics{\texttt{Filpud}( \bigwedge_{i}{\pred_i} )} & \assign & \bigsqcap_{i} {\asemantics{\texttt{Flipud}( \pred_i )}}  \\ \\ 
\end{array} 
&
\begin{array}{rll}
\asemantics{\texttt{Fliplr}( \emph{len}(e.\emph{size}) = c )} & \assign & \big( \emph{len}(e.\emph{size}) = c \big) \\ 
%\asemantics{\texttt{Fliplr}( e.\emph{size}[c_1] = c_2 )} & \assign & \big( e.\emph{size}[c_1] = c_2 \big) \\ 
\asemantics{\texttt{Fliplr}( \emph{len}(e.\emph{arr}) = c )} & \assign & \big( \emph{len}(e.\emph{arr}) = c \big) \\ 
%\asemantics{\texttt{Fliplr}( e.\emph{arr}[c_1] = c_2 )} & \assign & \emph{true} \\ 
\asemantics{\texttt{Fliplr}( e = c )} & \assign & \big( e = \semantics{\texttt{Fliplr}(c)} \big) \\ 
\asemantics{\texttt{Fliplr}( \bigwedge_{i}{\pred_i} )} & \assign & \bigsqcap_{i} {\asemantics{\texttt{Fliplr}( \pred_i )}}  \\ \\ 
\end{array}
\end{array}
\]
\caption{Abstract semantics for tensor reshaping DSL.}
\figlabel{matrixdslasemantics}
\end{figure}

